Relating by Contrasting: A Data-efficient Framework for Multimodal Generative Models

Multimodal learning for generative models often refers to the learning of abstract concepts from the commonality of information in multiple modalities, such as vision and language. While it has proven effective for learning generalisable representations, the training of such models often requires a large amount of "related" multimodal data that shares commonality, which can be expensive to come by. To mitigate this, we develop a novel contrastive framework for generative model learning, allowing us to train the model not just by the commonality between modalities, but by the distinction between "related" and "unrelated" multimodal data. We show in experiments that our method enables data-efficient multimodal learning on challenging datasets for various multimodal VAE models. We also show that under our proposed framework, the generative model can accurately identify related samples from unrelated ones, making it possible to make use of the plentiful unlabeled, unpaired multimodal data.

==> 1introduction_draft1.tex <==
\section{Introduction}
\label{sec:introduction}
%
The goal of disentanglement is to learn a generative model, whose latent is reflective of the ground-truth factor of variations of data \citep{tenenbaum2000separating, bengio2013representation}. 
%
% short:
%However, it has been shown that there is no guarantee that learned latent variables match the true generating factors under an unsupervised generative model learning scheme, where the only constraint is to optimise the marginal likelihood distribution.
%
Consider a data generation process $\x = g^\star (\s)$, where $\x$ denotes real data, $\s$ the factors of variation and $g^\star$ a deterministic function that defines the true generative model.
%
Existing techniques for disentangled representation learning aims to learn a generative model $\x = g_\theta(\z)$, whereby optimising $g_\theta$ to reconstruct $\x$, the hope is to also learn $\z$ that corresponds to the factors of variation in $\s$.
%
Unfortunately, this approach to disentanglement has been shown ineffective under an unsupervised scheme --- there is no guarantee that learned latent variables represent true generating factors by simply matching the marginal likelihood distributions \citep{hyvarinen2017nonlinear, locatello2019challenging, shu2020weakly} .

To tackle with this drawback, different forms of weak supervision in generative model learning are introduced, among them is multimodal learning.
%
Under this setting, one can observe multimodal pair $\left\{\x, \ \y\right\}$, where $\x$ and $\y$ are data from two different modalities that shares a subset of factors of variation $\s_c \subset \s$, and differs for all other factors $\s_p = \s \backslash \s_c$.
%
As a concrete example, consider a photo-sketch multimodal dataset $\{X,Y\}$ where each $\y \in Y$ is the line draw of corresponding photo $\x \in X$.
%
In the setting we just described, $\s_c$ controls the object/scene described by the image, while $\s_p$ describes the different styles of realistic photos and sketches.
%
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{images/pairedness_graph.png}
    \caption{
    %
    \textbf{\textit{Left:}} Past work on multimodal generative models hypothesises a generative process $g^\star$, where observations share one set of common factor $\s_c$.
    %
    The observations $\x$, $\y$ of the generative model $g_\theta$ therefore depends only on latent variable $\z$.
    %
    \textbf{\textit{Right:}} In this work, we assume that each modality is generated independently (like how most datasets are constructed independently) and that the common factor $\s_c$ is not necessarily shared, giving rise to an extra "pairedness" random variable $p$, where $p=1$ if $\s_c^{\x} = \s_c^{\y}$, $0$ otherwise.
    %
    In the generative model, $\x$, $\y$ now depends on both the latent variable $\z$ and the pairedness indicator $p$.
    % 
    In this work we make the simplifying assumption that the joint likelihood $p_\theta(\x,\y)$ should be high when $p=1$, and low otherwise, but other forms of dependency on $p$ can be taken.
    }
    \label{fig:graph}
\end{figure}
%
Recently, \cite{shi2019variational} showed quantitatively that the representations learned from leveraging the underlying commonality $\s_c$ --- under both their proposed MMVAE model and the MVAE model by \cite{MVAE_wu_2018} --- results in better representation learning compared to unsupervised (single-modal) \gls{VAE}.
%
% shorter version
%However, both frameworks require a large amount of paired multimodal data, which requires two labelled datasets, if not one-to-one correspondence between instances of the dataset.
% longer version
However, both approaches (and most multimodal \glspl{VAE}) require a large amount of multimodal data, which can be expensive to come by: 
%
constructing a multimodal dataset often requires labelled data, and in the case of more complicated multimodal scenarios such as language-vision, one-to-one or one-to-many correspondence between instances of the two datasets is required, as it is difficult to categorise the dataset in such a way that commonality among samples is preserved within categories.
%
Refer to \Cref{fig:cub-ex} for an example from CUB dataset (cite) --- the content of the two image-caption pairs are distinctly different even though they feature the same species of bird, making one-to-one correspondence between images and captions necessary.
%
\begin{wrapfigure}[7]{r}{0.21\textwidth}
    \vspace*{-1\baselineskip}
    \includegraphics[width=\linewidth]{images/cub_121_demo.png}
    \vspace{-1.5\baselineskip}
    \caption{Example}
    \label{fig:cub-ex}
\end{wrapfigure}

Luckily, not all hope is lost --- in any multimodal dataset, there exists an abundance of \emph{unpaired} multimodal sets $\left\{\x_i,\ \y_j \right\}$, where $i$, $j$ denotes the index of the datapoint and $\s_c^{\x_i} \neq \s_c^{\y_j}$ when $i \neq j$.
%
Our hope is to leverage these mismatched data that already exists in the dataset and train generative models via not just paired data, but the distinction between "paired" and "unpaired" multimodal observations.
%
Reasonably, this information is usually discarded in past work, as \emph{joint} multimodal data generation process is often assumed (see \Cref{fig:graph}, left).
%
Here, we take into account the fact that even though the world generates multimodal data jointly, each datasets are often collected \emph{independently}, resulting in cases of $\s_c^{\x_i} \neq \s_c^{\y_j}$.
%
The graph representation of our model can be found in \Cref{fig:graph} (right), where the "pairedness" between $\x$, $\y$ is considered as an observed random variable $p$, where $p=1$ when $\s_c^{\x}=\s_c^{\y}$ and $0$ otherwise.

While different forms of dependencies on $p$ can be taken, here we take the simplifying assumption that the joint marginal likelihood $p(\x,\y)$ should be high when $p=1$, and low when $p=0$.
%
This is achieved by optimising a \gls{NCE} loss \citep{gutmann2010noise}, which we show maximises the pointwise total correlation (PTC) between $\x$ and $\y$.
%
We demonstrate that this approach allows for the multimodal learning using only $10\%$ of the original data, and is effective across multiple datasets and different multimodal generative models;
%
furthermore, the application of NCE encourages a larger discrepancy between the marginal likelihoods of paired vs. unpaired data, which makes it possible to use the generative model as a classifier to find paired data in unlabelled multimodal dataset.
%
These data pairs can then be used for training to further improve the quality of the representations learned.


==> 1introduction_draft2.tex <==
\section{Introduction}
\label{sec:introduction}
%
\begin{wrapfigure}[9]{r}{0.25\textwidth}
    \vspace*{-1\baselineskip}
    \includegraphics[width=\linewidth]{images/cub_121_demo.png}
    \vspace{-1\baselineskip}
    \caption{Multimodal data from the CUB dataset}
    \label{fig:cub-ex}
\end{wrapfigure}
%
To comprehensively describe concepts in the real world, humans collect multiple cognitive signals of the same object such as image, sound, text and video. 
%
We refer to each of these media as \emph{modality}, and a collection of different media featuring the same underlying concept is characterised as \emph{multimodal} data.
%
Learning from multiple modalities has been shown to yield more generalisable representations\citep{zhang2020multimodal, guo2019deep, yildirim2014from}, as different modalities are often complimentary in content while overlapping for common abstract concept.
%
%The multimodal learning regime is also supported by human learning --- cognitive science research has shown that the association of information among multiple modalities benefits understanding and reasoning \citep{bauer1993diagrams,stein2009neural,quiroga2009explicit}.
%
%While multimodal learning comes naturally for us humans, training multimodal computational models requires a large amount of related multimodal data, which can be expensive to come by: 

Despite the motivation, it is worth noting that the multimodal framework is not exactly data-efficient---constructing a suitable dataset requires a lot of ``annotated'' unimodal data, as we need to ensure that each multimodal pair is related in a meaningful way.
%
The situation is worse when we consider more complicated multimodal settings such as language--vision, where one-to-one or one-to-many correspondence between instances of the two datasets are required, due to the difficulty in categorising data such that commonality amongst samples is preserved within categories.
%
See \Cref{fig:cub-ex} for an example from the CUB dataset \citep{cub}; although the same species of bird is featured in both image-caption pairs, their content differs considerably.
%
It would be unreasonable to apply the caption from one to describe the bird depicted in the other, necessitating one-to-one correspondence between images and captions.

However, the scope of multimodal learning has been limited to leveraging the commonality between ``related'' pairs, while largely ignoring ``unrelated'' samples potentially available in any multimodal dataset---constructed through random pairing between modalities (\cref{fig:r_vs_unr}).
%
We posit that if a distinction can be established between the ``related'' and ``unrelated'' observations within a multimodal dataset, we could greatly reduce the amount of related data required for effective learning.

\begin{wrapfigure}[10]{r}{0.25\textwidth}
    % \captionsetup[subfigure]{font=scriptsize}
    \vspace*{-0.5\baselineskip}
    \begin{subfigure}{.12\textwidth}
        \includegraphics[width=\linewidth]{images/intro_related.png}\vspace{-1.5pt}
        \caption{Related}\label{fig:intro_related}
    \end{subfigure}\hspace{2pt}
    \begin{subfigure}{.12\textwidth}
        \includegraphics[width=\linewidth]{images/intro_unrelated.png}\vspace{-1.5pt}
        \caption{Unrelated}\label{fig:intro_unrelated}
    \end{subfigure}
    \vspace{-6.5pt}
    \caption{Constructing related $\&$ unrelated samples}\label{fig:r_vs_unr}
\end{wrapfigure}
%
\Cref{fig:graph} formalises this proposal.
%
The multimodal generative process in previous work typically assumes that given a pair $(\x,\y)$, with $\x$, $\y$ being observations from different modalities, the pair \emph{always} shares a subset of factors of variation $\s_c \subset \s$ and differs for all other factors $\s_p = \s \backslash \s_c$ (\Cref{fig:graph}, left).
%
In this work, we introduce an additional random variable $r$ that dictates the ``relatedness'' between $\x$ and $\y$:
%
As seen in \Cref{fig:graph} (right), $r=1$ when $\s_c$ is shared and $0$ otherwise.

While different forms of dependencies on $r$ can be taken, here we make the simplifying assumption that the joint distibution $p(\x,\y)$ should be high when $r=1$, and low when $r=0$.
%
Intuitively, this can be achieved by adopting a max-margin metric.
%
We therefore propose to optimise the contrastive loss as introduced in \citep{hadsell2006dimensionality, triplet}, and demonstrate the effectiveness of the proposed framework from a few different perspectives: 
%
\begin{inparadesc}
    %
    \item[Improved multimodal learning:] showing improved multimodal learning for various state-of-the-art multimodal generative models on two challenging multimodal datasets.
    %
    This is evaluated on four different metrics \citep{shi2019variational} summarised in \Cref{sec:metrics};
    %
    \item[Data efficiency:] learning generative models under the contrastive framework requires only $20\%$ of the data needed in baseline methods to achieve similar performance---holding true across different models, datasets and metrics;
    % 
    \item[Label propagation:] the contrastive loss encourages a larger discrepency between related and unrelated data, making it possible to directly identify related samples using the~\gls{PTC} between observations.
    %
    We show that these data pairs can be used to further improve the learning of the generative model. 
    %
\end{inparadesc}
%
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{images/relatedness_graph.png}
    \caption{
    %
    \textbf{\textit{Left:}} Past work on multimodal generative models hypothesises a generative process $g^\star$, where observations share one set of common factor $\s_c$.
    %
    The observations $\x$, $\y$ of the generative model $g_\theta$ therefore depends only on latent variable $\z$.
    %
    \textbf{\textit{Right:}} In this work, we assume that each modality is generated independently (as most unimodal datasets are constructed independently) and that the common factor $\s_c$ is not necessarily shared, giving rise to an extra "relatedness" random variable $r$, where $r=1$ if $\s_c^{\x} = \s_c^{\y}$, $0$ otherwise.
    %
    In the generative model, $\x$, $\y$ now depends on both the latent variable $\z$ and the relatedness indicator $r$.
    % 
    In this work we make the simplifying assumption that the joint likelihood $p_\theta(\x,\y)$ should be high when $r=1$, and low otherwise, but other forms of dependency on $r$ can be taken.
    }
    \label{fig:graph}
\end{figure}
%

==> 3methods_draft1.tex <==


\section{Methodology}
%
\subsection{Multimodal VAE}
%
Given data over observations of $2$ modalties $\{\x, \y\}$, a \gls{VAE} can be employed to learn multi-modal generative model of the form $p_\Theta(\x, \y, \z) = p(\z) p_{\theta_x} (\x | \z) p_{\theta_y} (\y | \z)$, where $p_\theta(\cdot | \z)$ are deep neural networks (decoders) parametrised by $\Theta=\{\theta_x, \theta_y \}$.
%
To maximise joint marginal likelihood $\log p_\Theta(\x,\y)$, we can approximate the intractable true posterior by a variational posterior $q_\Phi(\z|\x,\y)$, allowing us to optimise an variational \gls{ELBO}, defined as
%
\begin{align}
  \log \p{\x, \y}
  \geq \Ex[\z \~ \q{\z \given \x, \y}]{\log \frac{\p{\z, \x, \y}}{\q{\z \given \x, \y}}}
  = -\mathcal{L}_v(\x,\y).
   \label{eq:elbo}
\end{align}

The remaining question here the approximated posterior $q_\Phi(\z|\x, \y)$ be modelled.
%
As mentioned in [previous work sec.], there are two schools of thinking:
%
\begin{enumerate}
    %
    \item Explicit joint model, where $q_\Phi$ is explicitly modelled by one joint encoder $q_\Phi(\z|\x,\y)$;
    
    \emph{Main drawback of this approach is that models are not able to handle missing input at test time, and often requires additional modelling components and inference steps.
    %
    This, as we will show, hinders the latent representation learning, and also significantly limits the complexity of multimodal data it can handle, limited to vision-vision only}
    % 
    \item Factorised joint model, where $q_\Phi$ is factorised as some combination $f$ of two unimodal encoders, i.e.     
    %
    \(
    \q{\z| \x,\y} =f\left(\q[\phi_x]{\z| \x} , \q[\phi_y]{\z | \y}\right).
    \)
    
    \emph{Two works we highlight here are MVAE \citep{MVAE_wu_2018} , where $f$ is defined as the \gls{PoE}, i.e.     
    %
    \(
    \q{\z| \x,\y} = \q[\phi_x]{\z| \x}\q[\phi_y]{\z | \y}
    \) 
    %
    and MMVAE \citep{shi2019variational} where $f$ is defined as the \gls{MoE}, i.e. 
    %
    \(
    \q{\z| \x,\y} = \frac{1}{2}\left(\q[\phi_x]{\z| \x} + \q[\phi_y]{\z | \y}\right).
    \)
    %
    }
\end{enumerate}

%
%    MVAE proposed by \citep{MVAE_wu_2018} is the first to allow for cross-modal generation ($\x \leftrightarrow \y$) without defining auxiliary single-modal \gls{VAE}, by defining the combination $f$ as the \gls{PoE}, i.e. $q_\Phi(\z|\x,\y) = q_{\phi_x}(\z|\x)q_{\phi_y}(\z|\y)$.
%

In this work, we will demonstrate the effectiveness of our approach for all these models, and for MMVAE, we show results not only on vision-vision, but also vision-language multimodal dataset.

\subsection{Motives for NCE}
%
Different to previous work where it is always assumed that $\x$ and $\y$ share commonality factor $s_c$ (\Cref{fig:graph}, left), we introduce an extra random variable $r$ that dictates the relatedness of $\x$ and $\y$, where $r=1$ when $s_c^x = s_c^y$, and $r=0$ otherwise (\Cref{fig:graph}, right).
%
In our work, we introduce an implicit form of dependency on $r$ by stating the following:
%
\begin{lemma}
%
Given two sets of observation $(\x_i,\y_j)$ and $(\x_i,\y_k)$, where $(\x_i,\y_j) \sim p_\Theta(\x,\y|\z_{ij})$, $\z_{ij}\sim q_\Theta(\z| r_{ij})$  and $(\x_i,\y_k) \sim p_\Theta(\x,\y|\z_{ik})$, $\z_{ik}\sim q_\Theta(\z| r_{ik})$.
%
If $r_{ij}=0$ and $r_{ik}=1$, then joint marginal likelihoods of the observations should satisfy $p(\x_i,\y_j)<p(\x_i,\y_k)$.
%
\end{lemma}
%
If our goal is to achieve data-efficient multimodal learning by utilising the information in $r$, according to Lemma 2.1, we can maximise the difference of joint marginal likelihoods between related and unrelated multimodal pairs.
%


Our starting point here is the \gls{CPC} as seen in (cite cpc, cite recon), which generally learns representations by learning to discriminate true observation of a particular representation from random ones.
%
Specifically, given an observation drawn from a batch of $N$ observations $\x \in X$, its corresponding representation $\c$ and some deterministic function $f_k$, the \gls{CPC} objective is defined as
%
\begin{align}\label{eq:nce_original}
        \L_N(\x, \bm{c}) = -  \log \frac{f_k(\x,\bm{c})}{\sum_{\x' \in X} f_k(\x', \bm{c})}.
\end{align}
%
where $\x'$ denotes "negative" samples randomly drawn from the batch $X$.
%
Intuitively, optimising \LN encourages $f_k(\x,\c)$ to be large when $\x$ is the corresponding observation of representation $\c$ (numerator), and small when $\x$ is a random sample from $X$ (denominator).
%
It has been shown that optimising \LN maximises the mutual information between $X$ and $C$ (cite CPC)
%and that the optimal value for $f_k(\x,\c)$ is given by $\frac{p(\x|\c)}{p(\x)}$. (cite CPC)

The \gls{CPC} objective can be adopted for multimodal generative models with minimal modification. 
%
Given a \emph{related} multimodal observation from a batch of $N$ observations  $\left\{\x,\y\right\} \in \left\{X, Y\right\}$, we can replace inputs to \LN in \cref{eq:nce_original} by $\x$, $\y$, yielding:
%
\begin{align}
        \mathcal{L}_N(\x, \y) &= \frac{1}{2}\left(\mathcal{L}_N(\y, \x) + \mathcal{L}_N(\x, \y) \right) \notag \\
        &= - \frac{1}{2}
            \log \frac{f_k(\x,\y)}{\sum_{\y' \in Y} f_k(\x, \y')} 
        - \frac{1}{2}
            \log \frac{f_k(\y,\x)}{\sum_{\x' \in X} f_k(\y, \x')} 
        \label{eq:nce_adopted}
\end{align}
% \begin{align}
%         \mathcal{L}_N(\x, \y) = 
%         - \log \frac{f_k(\x,\y)}{\sum_{\x' \in X} f_k(\x', \y)+\sum_{\y' \in Y} f_k(\x, \y')} 
%         \label{eq:nce_adopted}
% \end{align}
%
% \begin{wrapfigure}[11]{r}{0.21\textwidth}
%     \vspace*{-1\baselineskip}
%     \includegraphics[width=\linewidth]{images/intro_pretty.png}
%     \vspace*{-1.5\baselineskip}
%     \caption{\small Effect of \LN}
%     \label{fig:effect_obj}
% \end{wrapfigure}
% %
%
\begin{wrapfigure}[10]{r}{0.25\textwidth}
    \vspace*{-1\baselineskip}
    \begin{subfigure}{.12\textwidth}
        \includegraphics[width=\linewidth]{images/intro_related.png}
        \caption{related}\label{fig:intro_related}
    \end{subfigure}\hspace{1pt}
    \begin{subfigure}{.12\textwidth}
        \includegraphics[width=\linewidth]{images/intro_unrelated.png}
        \caption{Unrelated}\label{fig:intro_unrelated}
    \end{subfigure}
\end{wrapfigure}
%
Note that since NCE losses are asymmetrical, in \Cref{eq:nce_adopted} we have to take the average of two \glspl{NCE} to ensure negative samples in both modalities are equally accounted for.
% to ensure that the learning of different modalities is balanced.
%
With this objective, we can now maximise the mutual information between related samples.

One key question that remains is the choice of $f_k$.
%
There are two factors to consider, 
%
\begin{inparaenum}[1)]
%
\item $f_k$ should be large when $(\x, \y)$ are related and small when unrelated;
%
\item $f_k$ should be general enough so that the contrastive loss can be easily applied to different generative models, without needing extra inference components.
%
\end{inparaenum}

Taken these into account, the natural choice of $f_k$ is the joint marginal likelihood, $p_\Theta(\x,\y)$, which is approximated by \gls{ELBO}, $-\mathcal{L}_v(\x,\y)$, as seen in \cref{eq:elbo}.
%
Not only is $p_\Theta(\x,\y)$ larger when $\x$, $\y$ are related and smaller when unrelated, \gls{ELBO} is used in most \gls{VAE}-based generative model and can readily be used for the contrastive loss.
%
The \gls{NCE} loss can therefore be rewritten as
%
% \begin{align}
%         \mathcal{L}_N(\x, \y) 
%         &= - \log \frac{p_\Theta(\x,\y)}{\sum_{\x' \in X} p_\Theta(\x', \y)+\sum_{\y' \in Y} p_\Theta(\x, \y')} \notag \\
%         &= -\log p_\Theta(\x,\y) + \log(\sum_{\x' \in X} p_\Theta(\x', \y)+\sum_{\y' \in Y} p_\Theta(\x, \y')) \notag \\
%         & =  \mathcal{L}_v(\x, \y) -  \underset{\subalign{&\x_p=\x,\ \y_r \in Y or \\ &\x_p \in X,\ \y_r=\y}}{\text{\texttt{logsumexp}}} \ \mathcal{L}_v(\x_p, \y_r),
%         \label{eq:nce_op}
% \end{align}
%
\begin{align}
        \mathcal{L}_N(\x, \y) 
        &= - \frac{1}{2}
            \log \frac{p_\Theta(\x,\y)}{\sum_{\y' \in Y} p_\Theta(\x, \y')} 
        - \frac{1}{2}
            \log \frac{p_\Theta(\y,\x)}{\sum_{\x' \in X} p_\Theta(\y, \x')}  \notag \\
        &= -\log p_\Theta(\x,\y) + 
            \frac{1}{2} \left( 
                \log\sum_{\x' \in X} p_\Theta(\x', \y)+\log\sum_{\y' \in Y} p_\Theta(\x, \y') 
            \right) \notag \\
        & =  \mathcal{L}_v(\x, \y) -  
            \frac{1}{2} \left( \underset{\y' \in Y}{\text{\texttt{logsumexp}}} \ \mathcal{L}_v(\x, \y') +
            \underset{\x' \in X}{\text{\texttt{logsumexp}}} \ \mathcal{L}_v(\x', \y) \right)
        \label{eq:nce_op}
\end{align}
%
where the \texttt{logsumexp} operation calculates sum within $\log$ by computing the log of summed exponentials of inputs\footnote{Numerically stablised computation is available at \texttt{torch.logsumexp()} in PyTorch environment.}.
%
This loss then effectively maximises the difference between $p_\Theta(\x,\y)$ when $\x$, $\y$ are related vs. when they are unrelated, as illustrated in \Cref{fig:effect_obj}.
%
We also show that with $f_k$ approximating the joint marginal likelihood, optimising this loss maximises the Pointwise Total Correlation PTC$(\x,\y)$. 
%
See Appendix for derivation.

Note that even though \cref{eq:nce_op} contains the \gls{ELBO} objective, \LN by itself is not a effective objective for generative model training.
%
%This is because there are many different ways for the generative model to generate "bad" samples with low joint marginal likelihood, and yet high marginal likelihood can almost \emph{only} be achieved by accurately reconstructing the samples.
This is because it is much easier for the model to generate samples with low marginal likelihoods than those with high likelihoods.
%
Take \Cref{fig:llik} as an example --- for both MNIST (citemnist) and SVHN (cite svhn), high likelihood on distribution centered at $\x$ requires somewhat accurate reconstruction of the original image (i.e. $\hat{\x}$); 
%
\begin{wrapfigure}[13]{r}{0.4\textwidth}
    \vspace*{-0.4\baselineskip}
    \includegraphics[width=\linewidth]{images/llik.png}
    \vspace*{-1.5\baselineskip}
    \caption{\small Per-pixel log-likelihoods evaluated on a Normal distribution centered at $\x$ with constant variance, including (from left to right) original $\x$, reconstruction $\hat{\x}$, other digit $\x'$, other digit $\x''$ and random noise.}
    \label{fig:llik}
\end{wrapfigure}
%
on the other hand, both different digits ($\x'$ and $\x''$) and \textit{noise} results in very low likelihood. 
%
The takeaway here is --- it is trivial to optimise \cref{eq:nce_op} by minimising the second term instead of maximising the first.
%
We show in our experiments that optimising \cref{eq:nce_op} only will cause the model to stuck in a local minimum and generate random noise.

Due to the above analysis, we propose to use the \gls{NCE} loss in addition to the original \gls{ELBO} loss as a mutual information regularisation, arriving at our final objective
%
\begin{align}
    \L(\x, \y) = \mathcal{L}_v(\x, \y) + \LN(\x,\y).
\end{align}
%
Note that this objective can be generalised to situation where more than $2$ modalities are presented.
%
See Appendix for more details.

==> 3methods_neurips.tex <==


\section{Methodology} \label{sec:methodology}
%
Given data over observations from two modalties $(\x, \y)$, one can learn a
multimodal \gls{VAE} by optimising $p_\Theta(\x, \y, \z) = p(\z) p_{\theta_x} (\x | \z) p_{\theta_y} (\y | \z)$, where $p_\theta(\cdot | \z)$ are deep neural networks (decoders) parametrised by $\Theta=\{\theta_x, \theta_y \}$.
%
To maximise joint marginal likelihood $\log p_\Theta(\x,\y)$, one approximates
the intractable model posterior $p_\Theta(\z|\x,\y)$ with a variational posterior $q_\Phi(\z|\x,\y)$, allowing us to optimise an variational \gls{ELBO}, defined as
%
\begin{align}
  \log \p{\x, \y}
  \geq \Ex[\z \~ \q{\z \given \x, \y}]{\log \frac{\p{\z, \x, \y}}{\q{\z \given \x, \y}}}
  = \text{ELBO}(\x,\y).
   \label{eq:elbo}
\end{align}

The remaining question here the approximated posterior $q_\Phi(\z|\x, \y)$ be modelled.
%
As mentioned in \Cref{sec:background}, there are two schools of thinking, namely \emph{explicit joint model} such as JMVAE \citep{JMVAE_suzuki_1611} and \emph{factorised joint model} including MVAE \citep{MVAE_wu_2018} and MMVAE \citep{shi2019variational}.
%
In this work we demonstrate the effectiveness of our approach for all these models.

\subsection{Contrastive loss for "relatedness" learning}
%
Unlike previous work where it is always assumed that $\x$ and $\y$ are related (\Cref{fig:previous}), we introduce an extra random variable $r$ that dictates the \emph{relatedness} of multimodal observations (\Cref{fig:ours}), where $r=1$ when $\x$, $\y$ shares a pre-determined commonality (such as digit), and $r=0$ otherwise.
%
% Given generative model of the form $p_\Theta(\x,\y,\z,r)$ as shown in \Cref{fig:graph} (right) implicit dependency on $r$ can be established by observing the following:
%
To motivate our approach, we begin with the following hypothesis regarding the relationship between pointwise mutual information of related and unrelated observations of different modalities:
%
\begin{hypothesis}\label{hypo}
Let $(\x, \y) \sim p_\Theta(\x, \y)$ be a related data pair from two modalities, and let $\y'$ denote a data point not related with $\x$. %, i.e.\ with $(\x, \y') \sim p_\Theta(\x,\y| r=0)$.
%
Then we assume the pointwise mutual information $I(\x, \y) > I(\x, \y')$.
%\todo{We might want to make the weaker assumption that this is "usually" true, instead of for all $\x, \y, \y'$.}
\end{hypothesis}
%
Here we take $p_\Theta$ to refer to the multimodal objective in Eq.~\eqref{eq:elbo}, i.e.\ conditioning on $r=1$.
%
Pointwise mutual information provides a measure of the statistical dependence between two values $a, b$, and for a joint distribution
$p(a, b)$ is defined as
%\begin{align}
\(I(a, b) = \log \frac{p(a, b)} {p(a)p(b)}\);
%\end{align}
%
%$p(a, b | c)$ is defined as
% \begin{align}
% I(a, b | c) = \log \frac{p(a, b | c)} {p(a | c)p(b|c)}
% \end{align}
%
%It differs from the more common notion of mutual information by measuring dependency specifically at two \textit{values};
mutual information is the expected value of the pointwise mutual information under $p(a, b)$.
%
The assumption in Hypothesis~\ref{hypo} should be fairly uncontroversial: we say simply that under the joint distribution for related data $p_\Theta(\x, \y)$, dependence measured between related points $\x, \y$ is stronger than between unrelated points $\x, \y'$.

In practical terms, we can use this formulation of dependence to motivate a contrastive loss.
%
For related $\x, \y$ and unrelated $\x, \y'$, we can expand the inequality $I(\x, \y) > I(\x, \y')$ as
\begin{align*}
\log p_\Theta(\x, \y) - \log p_\Theta(\x) - \log p_\Theta(\y)
>
\log p_\Theta(\x, \y') - \log p_\Theta(\x) - \log p_\Theta(\y').
\end{align*}
%
% where we have made the additional assumption that the marginal distributions over $\x$ becomes independent of $r$ once $\y$ is integrated out, and vice versa. \todo{Justify this somehow?}
% From the dependency structure in Fig.~\ref{fig:graph}, we note that the marginals over $\x$ and $\y$ do not depend on the value of $r$, as $r$ only
Re-arranging terms, we introduce an explicit slack variable $C > 0$, and write
\begin{align}
\log p_\Theta(\x, \y) - \log p_\Theta(\x, \y')
&=
 \underbrace{[\log p_\Theta(\y) - \log p_\Theta(\y')]}_{\text{1. marginal prevalence term}} \ + \underbrace{C}_{\vphantom{[\log p_\Theta(\y) - \log p_\Theta(\y')]}\text{2.unrelated instance gap}}.\label{eq:diff}
\end{align}
%
Intuitively, this can be understood as decomposing the difference between the two joint probabilities $\log p_\Theta(\x, \y)$ and $\log p_\Theta(\x, \y')$ as two terms:
%
1. $[\log p_\Theta(\y) - \log p_\Theta(\y')]$, which captures the difference in the joint probabilities due to the marginal contribution of the different values of $\y$ and $\y'$, a term irrelevant to whether the data are related;
%
and 2. $C$, which captures the remaining gap in joint probabilities due to evaluating related as opposed to unrelated points.
%
\begin{wrapfigure}[11]{l}{0.23\textwidth}
    \captionsetup[subfigure]{font=scriptsize}
    \vspace*{-0.7\baselineskip}
    \begin{subfigure}{.47\linewidth}
        \includegraphics[width=\linewidth]{images/intro_related.png}\vspace{-1.5pt}
        \caption{Related}\label{fig:intro_related}
    \end{subfigure}\hspace{2pt}
    \begin{subfigure}{.47\linewidth}
        \includegraphics[width=\linewidth]{images/intro_unrelated.png}\vspace{-1.5pt}
        \caption{Unrelated}\label{fig:intro_unrelated}
    \end{subfigure}
    \vspace{-6.5pt}
    \caption{Constructing related $\&$ unrelated samples}\label{fig:r_vs_unr}
\end{wrapfigure}
%
The above suggests that to achieve data-efficient multimodal learning by utilising the relatedness between multimodal pairs, one may maximise term (2) in \Cref{eq:diff} through maximising the difference between the joint marginal likelihood of related pairs $p_\Theta(\x,\y)$ (\Cref{fig:intro_related}) and that of unrelated pairs $p_\Theta(\x,\y')$ (\Cref{fig:intro_unrelated}).
%
This poses multimodal learning as a max-margin optimisation problem, for which a
natural choice of objective is the contrastive (triplet) loss $\mathcal{L}_c$ that takes the following form:
%
\begin{align}\label{eq:nce_original}
        \L_C(\x, \y, \y') = d(\x,\y)- d(\x,\y')+m.
\end{align}
%
Intuitively, \LC attempts to make distance $d$ between a positive pair $(\x,\y)$ smaller than the distance between a negative pair $(\x,\y')$ by margin $m$.
%
We can then adopt this loss to our relatedness learning objective by replacing $d$ by (negative) joint marginal likelihood $\log p_\Theta$, which is approximated by \gls{ELBO} as shown in \Cref{eq:elbo}.
%
Further, we can follow the practice in \cite{song2016deep} and take the \texttt{LogSumExp} among $N$ negative samples $y'_i\in \{Y\}_{i=1}^N$, giving us the following objective
%
\begin{align}\label{eq:nce_half}
    \L_C(\x, Y) = -\log p_\Theta(\x,\y) + \log \sum_{i=1}^N p_\Theta(\x,\y'_i).
\end{align}
%
Also, since the loss is asymmetric, one can average over $\L_C(\y, X)$ and $\L_C(\x, Y)$  so that negative samples in both modalities are accounted for.
%
We can now write our final contrastive objective:

\vspace{-8pt}
\scalebox{0.91}{%
\begin{minipage}{1.0\linewidth}
\begin{align}
  \mathcal{L}_C(\x, \y)
  &=  \frac{1}{2} \left\{ \mathcal{L}_C(\x,Y) + \mathcal{L}_C(\y, X) \right\}
  =
  -\log p_\Theta(\x,\y) +
  \frac{1}{2} \left(
          \log\sum_{\x'_i = 1}^N p_\Theta(\x', \y)+\log\sum_{\y'_i = 1}^N p_\Theta(\x, \y')
      \right) \notag\\
  &\approx
  \underbrace{
      \vphantom{
          \frac{1}{2} \left(
              \underset{\x' \in X}{\text{\texttt{logsumexp}}} \ \text{ELBO}(\x', \y) +
              \underset{\y' \in Y}{\text{\texttt{logsumexp}}} \ \text{ELBO}(\x, \y') \right)
      }- \text{ELBO}(\x, \y)}_{\text{\circled{1}}} +
      \underbrace{
          \frac{1}{2} \left(
              \underset{\x' \in X}{\text{\texttt{logsumexp}}} \ \text{ELBO}(\x', \y) +
              \underset{\y' \in Y}{\text{\texttt{logsumexp}}} \ \text{ELBO}(\x, \y')  \right)
      }_{\text{\circled{2}}}
  \label{eq:nce_op}
\end{align}
\end{minipage}}

% where $\L_v$ is negative \gls{ELBO} as seen in \Cref{eq:elbo}, and the \texttt{logsumexp} operation calculates sum within $\log$ by computing the log of summed exponentials of inputs\footnote{Numerically stablised computation is available at \texttt{torch.logsumexp()} in PyTorch environment.}.
%
Note that since only \gls{ELBO} terms are needed in \Cref{eq:nce_op}, the contrastive learning framework can be directly applied to \emph{any} multimodal generative model without needing extra components.
%
In our experiments, we take $N=5$ negative samples for each modality.
%
We also show that it is possible to apply the contrastive loss for cases where number of modalities considered is greater than $2$.
%
See \Cref{sec:m>2} for more details.

% \paragraph{Benefits}
% The benefits of using the contrastive loss are threefold.
% %
% First, the contrastive loss effectively utilises the \emph{relatedness} information, which not only enables data-efficient multimodal learning [CITE EXPERIMENT], but also provides an accurate prediction for the relatedness of unlabelled multimodal pairs;
% %
% it is also theoretically grounded -- in \cite{cpc}, authors showed that optimising \LC maximises the mutual information between its inputs, in our case, related multimodal pair $(\x,\y)$.
% %
% We also show that for our specific formulation of \LC maximises the \gls{PTC} between $(\x,\y)$, which is defined as $\text{PTC}(\x,\y)=\log\left( p_\Theta(\x,\y)/p_{\theta_x}(\x)p_{\theta_y}(\y)\right)$;
% %
% lastly, since only \gls{ELBO} terms are needed in \Cref{eq:nce_op}, the contrastive learning framework can be directly applied to any multimodal generative models without needing extra inference components.
%
\begin{wrapfigure}[7]{r}{0.3\textwidth}
    \vspace*{-1.9\baselineskip}
    \centering
    \includegraphics[width=\linewidth]{images/llik.png}
    \vspace*{-1.5\baselineskip}
    \caption{\small $\log p(\x,\y)$ of imitation, unrelated digits and random noise, where $p=\mathcal{N}(\bm{m_x}, \bm{m_y})$.}
    \label{fig:llik}
\end{wrapfigure}
%
\paragraph{Dissecting \LC}
%
Although \cref{eq:nce_op} directly maximises \gls{ELBO} like the \gls{VAE} through {\footnotesize \circled{1}}, \LC by itself is not a effective objective for \gls{VAE} training since \LC also contains term {\footnotesize \circled{2}} that \emph{minimises} \gls{ELBO}, which can overpower the effect of {\footnotesize \circled{1}} during training.

We provide an intuition to this phenomenon using a simple Gaussian example, illustrated in \Cref{fig:llik}.
%
Here, we evaluate the log likelihood of $\log p(\x,\y)$ in column 2, 3, 4 (green) on a Gaussian distribution $\mathcal{N}((\bm{m_x},\bm{m_y}); c)$, with the images in the first column of \Cref{fig:llik} as means and with constant variance $c$.
%
We can see that while achieving high log likelihood $\log p(\x,\y)$ on this distribution requires close imitation of $(\bm{m_x},\bm{m_y})$ (second column), both unrelated digits (third column) and noise (last column) can lead to equally low joint log likelihoods.
%
This indicates that the generative model need not generate valid, unrelated images to minimise {\footnotesize \circled{2}}---generating noise would have the same effect on log likelihood.
%
As a result, the model can trivially minimise minimise \LC by generating noise that minimises {\footnotesize \circled{2}} instead of accurate reconstruction that maximises {\footnotesize \circled{1}}.

This learning dynamic is verified empirically, as we show in \Cref{fig:loss_gamma0} in \Cref{sec:ineffectiveness}:
%
if we optimise \LC by itself, while the loss approaches 0 within the first 100 iterations, both {\footnotesize \circled{1}} and {\footnotesize \circled{2}} takes on extremely low values, resulting in a model that generates random noise.

\paragraph{Final objective}
%
To mitigate the above effect, we need to ensure that when optimising the objective in \Cref{eq:nce_op}, minimising {\footnotesize \circled{2}} does not overpower maximising {\footnotesize \circled{1}}.
%
We therefore introduce a hyperparameter $\gamma$ on {\footnotesize \circled{1}} to upweight the maximisation of \gls{ELBO}.
%
Our final objective is therefore:
%
\begin{align}
    \mathcal{L}(\x, \y) =
    - \gamma \text{ELBO}(\x, \y) +
    \frac{1}{2} \left(
        \underset{\x' \in X}{\text{\texttt{logsumexp}}} \ \text{ELBO}(\x', \y) +
        \underset{\y' \in Y}{\text{\texttt{logsumexp}}} \ \text{ELBO}(\x, \y')  \right),
    \label{eq:final}
\end{align}
%
where $\gamma>1$.
%
In our experiments we simply take $\gamma=2$ (upweight \gls{ELBO} in \LC by 1), however as observed in our ablation studies (see \Cref{sec:gamma}), larger $\gamma$ encourages better quality of generation and more stable training in some cases, while models trained with smaller $\gamma$ are better at predicting ``relatedness'' between multimodal samples.
%
We also note that optimising \Cref{eq:final} maximises $\text{PTC}(\x,\y)=\log\left( p_\Theta(\x,\y)/p_{\theta_x}(\x)p_{\theta_y}(\y)\right)$;
%
see \Cref{sec:ptc} for a proof.

\subsection{Estimating $p(\x,\y)$}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> broaderimpact.tex <==
\section{Broader Impact}

As discussed thoroughly in our paper, our proposed contrastive framework improves the performance of wide range of multimodal generative models, and can by extension be applied to a variety of multimodal scenarios these models are designed for.
%
This includes vision-language, audio-video, sketch-photo, 2D-3D, sensor fusion, and so on \citep{zhang2020multimodal,guo2019deep}.

%Many existing work on multimodal deep generative models are inspired by exploring human-like learning.
%
Multimodal generative models have strong ties to explainable AI, especially if any of the modalities used are in perceptual domain, since the generation of one modality can then be used to explain another.
%
Being able to provide explanation is not only essential to increasing the societal acceptance of decision-making by algorithms, but also required as per the "right to explanation" clause in the EU General Data Protection Regulation (GDPR).
%
However, any technology can be problematic when misused.
%
When the data used involves human characteristics such as face, speech, ethnicity and gender/sex, multimodal generation can be a dangerously effective tool for police or government surveillance, raising significant security and privacy concerns, and cause for regulation.

Many existing works on multimodal learning were inspired by how humans learn from multiple modalities in the real world.
%
While these motivations are valid from a theoretical standpoint, they are inconsistent to the reality of machine learning, where the data collection processes are mostly unimodal.
%
Constructing multimodal datasets therefore relies heavily on detailed annotations of these datasets, and can therefore only be used by those who has the resources to collect them. 
%
In the talk delivered by \citeauthor{kalluri_2019} at NeurIPS 2019, the speaker noted the importance to consider how one's work could shift the power in society from those who possesses them to those who don't.
%
With this in mind, our work is driven by improving the data efficiency in multimodal learning, making the implementation of multimodal algorithms on real world tasks more accessible to those with less resources.



Despite the distinct improvements in data-efficiency, we must also admit that there are trade-offs in terms of computational efficiency.
%
However, our best performing model in the most complicated dataset (contrastive MMVAE, on CUB) uses around 5GB memory, which can be comfortably fit into a modern GPU.
%
To mitigate this trade-off in processing power, future work can look into the possibility of using "relatedness" in a non-contrastive way, possibly by explicitly define it in the graphical model.
%
%We also encourage the research community to collect multimodal data when convenient, for instance audio accompanying the video in action recognition dataset, or 



